Energy-Efficient Routing for Electric Vehicles under Acceleration and Load Effects

This paper proposes an Acceleration and Load-Dependent Electric Vehicle Routing Problem (ALD-EVRP), to optimize the energy consumption (EC) while capturing the effects of changing traffic conditions between peak and off-peak periods. We generalize the time-dependent speed model by replacing step functions with piecewise linear functions. The EC of each vehicle is influenced by its speed, acceleration, and real-time load. A mathematical model is developed and solved using BonMin, and a custom meta-heuristic algorithm is proposed for large-scale problems, yielding the same results as BonMin on small problems and performing better on larger ones. This is validated with real data from Singapore.

==> table/full2.tex <==
% % \usepackage{caption}
% % \usepackage{multirow}
% % \usepackage{booktabs}


% \begin{table}[t]
% \caption{Result details on real-world instances with multiple vehicles}
% \label{tab:full2}
% \centering
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{rrrrrlrr|lrrrrrlr} 
% \toprule
% \multicolumn{1}{c}{\textbf{\textbf{Ins}}} & \multicolumn{1}{c}{\textbf{\textbf{n}}} & \multicolumn{1}{c}{$W_{\mathrm{Best}}$} & \multicolumn{1}{c}{TT} & \multicolumn{1}{c}{$N_{\mathrm{veh}}$} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Gap}                  & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{\textbf{Ins}}} & \multicolumn{1}{c}{\textbf{\textbf{n}}} & \multicolumn{1}{c}{$W_{\mathrm{Best}}$} & \multicolumn{1}{c}{TT} & \multicolumn{1}{c}{$N_{\mathrm{veh}}$} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Gap}  \\ 
% \cline{1-7}\cline{9-16}
% \textbf{001}                              & 30                                      & 517857.06                               & 853.88                 & 9                                      &                      & \textbf{0.00}                            &                       &                      & \textbf{032}                              & 87                                      & 1205223.46                              & 2011.92                & 20                                     &                      & 0.81                     \\
% \textbf{002}                              & 41                                      & 696986.63                               & 1157.34                & 12                                     &                      & \textbf{\textbf{0.00}}                   &                       &                      & \textbf{033}                              & 87                                      & 1053836.57                              & 1747.60                & 18                                     &                      & 0.77                     \\
% \textbf{003}                              & 43                                      & 524189.38                               & 868.39                 & 9                                      &                      & \textbf{\textbf{0.00}}                   &                       &                      & \textbf{034}                              & 87                                      & 1399988.53                              & 2308.77                & 24                                     &                      & 0.76                     \\
% \textbf{004}                              & 44                                      & 766585.00                               & 1306.23                & 12                                     &                      & \textbf{\textbf{0.00}}                   &                       &                      & \textbf{035}                              & 88                                      & 1068404.97                              & 1783.02                & 18                                     &                      & 0.82                     \\
% \textbf{005}                              & 51                                      & 1001786.61                              & 1668.24                & 17                                     &                      & \textbf{\textbf{0.00}}                   &                       &                      & \textbf{036}                              & 90                                      & 1276698.42                              & 2106.07                & 22                                     &                      & 0.93                     \\
% \textbf{006}                              & 53                                      & 633356.04                               & 1075.81                & 10                                     &                      & \textbf{\textbf{\textbf{\textbf{0.00}}}} &                       &                      & \textbf{037}                              & 91                                      & 1206481.57                              & 2021.59                & 20                                     &                      & 0.99                     \\
% \textbf{007}                              & 54                                      & 496666.94                               & 839.766                & 8                                      &                      & \textbf{\textbf{\textbf{\textbf{0.00}}}} &                       &                      & \textbf{038}                              & 93                                      & 941496.96                               & 1551.38                & 16                                     &                      & 1.15                     \\
% \textbf{008}                              & 57                                      & 879079.49                               & 1464.67                & 15                                     &                      & \textbf{\textbf{0.00}}                   &                       &                      & \textbf{039}                              & 98                                      & 1531762.13                              & 2544.85                & 26                                     &                      & 1.30                     \\
% \textbf{009}                              & 59                                      & 639686.61                               & 1059.10                & 11                                     &                      & 0.01                                     &                       &                      & \textbf{040}                              & 98                                      & 1692423.57                              & 2839.44                & 28                                     &                      & 1.28                     \\
% \textbf{010}                              & 60                                      & 1067694.06                              & 1739.68                & 19                                     &                      & 0.06                                     &                       &                      & \textbf{041}                              & 104                                     & 1120009.66                              & 1870.06                & 19                                     &                      & 1.53                     \\
% \textbf{011}                              & 61                                      & 937753.26                               & ~1552.20               & 16                                     &                      & 0.04                                     &                       &                      & \textbf{042}                              & 105                                     & 1400651.05                              & 2343.46                & 24                                     &                      & 0.80                     \\
% \textbf{012}                              & 62                                      & 693719.93                               & 1153.84                & 12                                     &                      & 0.07                                     &                       &                      & \textbf{043}                              & 106                                     & 1416699.78                              & 2347.57                & 24                                     &                      & 1.69                     \\
% \textbf{013}                              & 64                                      & 990999.71                               & 1637.26                & 17                                     &                      & 0.09                                     &                       &                      & \textbf{044}                              & 110                                     & 1021367.59                              & 1681.60                & 18                                     &                      & 1.91                     \\
% \textbf{014}                              & 64                                      & 1082607.11                              & 1811.89                & 18                                     &                      & 0.11                                     &                       &                      & \textbf{045}                              & 110                                     & 1178598.16                              & 2434.90                & 21                                     &                      & 2.15                     \\
% \textbf{015}                              & 65                                      & 937852.26                               & 1559.22                & 16                                     &                      & 0.14                                     &                       &                      & \textbf{046}                              & 110                                     & 1534117.14                              & 2592.52                & 25                                     &                      & 2.30                     \\
% \textbf{016}                              & 66                                      & 784678.40                               & 1277.09                & 14                                     &                      & 0.17                                     &                       &                      & \textbf{047}                              & 114                                     & 1306986.80                              & 2197.36                & 22                                     &                      & 2.73                     \\
% \textbf{017}                              & 68                                      & 1128448.08                              & 1881.16                & 19                                     &                      & 0.17                                     &                       &                      & \textbf{048}                              & 115                                     & 1545978.28                              & 2566.18                & 26                                     &                      & 2.73                     \\
% \textbf{018}                              & 71                                      & 1080590.08                              & 1803.08                & 18                                     &                      & 0.20                                     &                       &                      & \textbf{049}                              & 116                                     & 1294564.47                              & 1783.39                & 23                                     &                      & 2.87                     \\
% \textbf{019}                              & 75                                      & 1004208.40                              & 1676.43                & 17                                     &                      & 0.21                                     &                       &                      & \textbf{050}                              & 117                                     & 1550340.75                              & 2576.26                & 27                                     &                      & 2.85                     \\
% \textbf{020}                              & 76                                      & 850835.70                               & 1438.11                & 14                                     &                      & 0.25                                     &                       &                      & \textbf{051}                              & 119                                     & 1489288.28                              & 2488.27                & 25                                     &                      & 3.00                     \\
% \textbf{021}                              & 77                                      & 1003736.90                              & 1668.44                & 17                                     &                      & 0.29                                     &                       &                      & \textbf{052}                              & 121                                     & 1437003.39                              & 2363.84                & 25                                     &                      & 3.14                     \\
% \textbf{022}                              & 79                                      & 1024441.49                              & 1744.07                & 16                                     &                      & 0.31                                     &                       &                      & \textbf{053}                              & 121                                     & 1620065.26                              & 2669.71                & 28                                     &                      & 2.92                     \\
% \textbf{023}                              & 80                                      & 1006551.22                              & 1675.72                & 17                                     &                      & 0.38                                     &                       &                      & \textbf{054}                              & 123                                     & 1644541.98                              & 2792.57                & 27                                     &                      & 3.45                     \\
% \textbf{024}                              & 80                                      & 1347631.55                              & 2265.40                & 22                                     &                      & 0.36                                     &                       &                      & \textbf{055}                              & 127                                     & 1294030.20                              & 2192.21                & 22                                     &                      & 3.99                     \\
% \textbf{025}                              & 81                                      & 973430.19                               & 1600.14                & 17                                     &                      & 0.37                                     &                       &                      & \textbf{056}                              & 128                                     & 1955192.84                              & 3261.98                & 33                                     &                      & 4.33                     \\
% \textbf{026}                              & 82                                      & 955683.62                               & 1608.56                & 16                                     &                      & 0.41                                     &                       &                      & \textbf{057}                              & 129                                     & 1837813.30                              & 3033.64                & 32                                     &                      & 4.95                     \\
% \textbf{027}                              & 82                                      & 1053831.34                              & 1740.97                & 18                                     &                      & 0.50                                     &                       &                      & \textbf{058}                              & 135                                     & 1695431.80                              & 2859.04                & 28                                     &                      & 5.36                     \\
% \textbf{028}                              & 82                                      & 1039985.22                              & 1717.50                & 18                                     &                      & 0.44                                     &                       &                      & \textbf{059}                              & 136                                     & 1649242.21                              & 2745.27                & 28                                     &                      & 5.21                     \\
% \textbf{029}                              & 85                                      & 1252397.61                              & 2123.76                & 20                                     &                      & 0.61                                     &                       &                      & \textbf{060}                              & 143                                     & 1708512.35                              & 2839.09                & 29                                     &                      & 4.60                     \\
% \textbf{030}                              & 85                                      & 1315005.32                              & 2231.53                & 21                                     &                      & 0.63                                     &                       &                      & \textbf{061}                              & 145                                     & 1954030.69                              & 3237.25                & 34                                     &                      & 5.03                     \\
% \textbf{031}                              & 86                                      & 1349636.77                              & 2251.47                & 23                                     &                      & 0.74                                     &                       &                      & \textbf{062}                              & 165                                     & 2512379.48                              & 4166.04                & 43                                     &                      & 5.24                     \\ 
% \hline\hline
% \textbf{Avg}                              & \textbf{67}                             & \textbf{936706.84}                      & \textbf{1562.93}       & \textbf{15.7}                          & \multicolumn{1}{r}{} & \textbf{0.21}                            &                       & \multicolumn{1}{r}{} & \textbf{Avg}                              & \textbf{113}                            & \textbf{1469134.25}                     & \textbf{2450.22}      & \textbf{25}                           & \multicolumn{1}{r}{} & \textbf{2.63}           \\
% \bottomrule
% \end{tabular}
% }
% \end{table} 


\begin{table}[t]
\caption{Result details on real-world instances with multiple vehicles (Part 1)}
\label{tab:full2a}
\centering
\scriptsize % 调小字体
\resizebox{\columnwidth}{!}{
\begin{tabular}{rrrrrlr} 
\toprule
\multicolumn{1}{c}{\textbf{Ins}} & \multicolumn{1}{c}{\textbf{n}} & \multicolumn{1}{c}{$W_{Best}$} & \multicolumn{1}{c}{TT} & \multicolumn{1}{c}{$N_{veh}$} &  & \multicolumn{1}{c}{Gap}  \\ 
\midrule
\textbf{001} & 30  & 517857.06  & 853.88  & 9  & & \textbf{0.00} \\
\textbf{002} & 41  & 696986.63  & 1157.34 & 12 & & \textbf{0.00} \\
\textbf{003} & 43  & 524189.38  & 868.39  & 9  & & \textbf{0.00} \\
\textbf{004} & 44  & 766585.00  & 1306.23 & 12 & & \textbf{0.00} \\
\textbf{005} & 51  & 1001786.61 & 1668.24 & 17 & & \textbf{0.00} \\
\textbf{006} & 53  & 633356.04  & 1075.81 & 10 & & \textbf{0.00} \\
\textbf{007} & 54  & 496666.94  & 839.77  & 8  & & \textbf{0.00} \\
\textbf{008} & 57  & 879079.49  & 1464.67 & 15 & & \textbf{0.00} \\
\textbf{009} & 59  & 639686.61  & 1059.10 & 11 & & 0.01 \\
\textbf{010} & 60  & 1067694.06 & 1739.68 & 19 & & 0.06 \\
\textbf{011} & 61  & 937753.26  & 1552.20 & 16 & & 0.04 \\
\textbf{012} & 62  & 693719.93  & 1153.84 & 12 & & 0.07 \\
\textbf{013} & 64  & 990999.71  & 1637.26 & 17 & & 0.09 \\
\textbf{014} & 64  & 1082607.11 & 1811.89 & 18 & & 0.11 \\
\textbf{015} & 65  & 937852.26  & 1559.22 & 16 & & 0.14 \\
\textbf{016} & 66  & 784678.40  & 1277.09 & 14 & & 0.17 \\
\textbf{017} & 68  & 1128448.08 & 1881.16 & 19 & & 0.17 \\
\textbf{018} & 71  & 1080590.08 & 1803.08 & 18 & & 0.20 \\
\textbf{019} & 75  & 1004208.40 & 1676.43 & 17 & & 0.21 \\
\textbf{020} & 76  & 850835.70  & 1438.11 & 14 & & 0.25 \\
\textbf{021} & 77  & 1003736.90 & 1668.44 & 17 & & 0.29 \\
\textbf{022} & 79  & 1024441.49 & 1744.07 & 16 & & 0.31 \\
\textbf{023} & 80  & 1006551.22 & 1675.72 & 17 & & 0.38 \\
\textbf{024} & 80  & 1347631.55 & 2265.40 & 22 & & 0.36 \\
\textbf{025} & 81  & 973430.19  & 1600.14 & 17 & & 0.37 \\
\textbf{026} & 82  & 955683.62  & 1608.56 & 16 & & 0.41 \\
\textbf{027} & 82  & 1053831.34 & 1740.97 & 18 & & 0.50 \\
\textbf{028} & 82  & 1039985.22 & 1717.50 & 18 & & 0.44 \\
\textbf{029} & 85  & 1252397.61 & 2123.76 & 20 & & 0.61 \\
\textbf{030} & 85  & 1315005.32 & 2231.53 & 21 & & 0.63 \\
\textbf{031} & 86  & 1349636.77 & 2251.47 & 23 & & 0.74 \\ 
\midrule
\textbf{Avg} & \textbf{67} & \textbf{936706.84} & \textbf{1562.93} & \textbf{15.7} & & \textbf{0.21} \\
\bottomrule
\end{tabular}}
\end{table}


\begin{table}[t]
\caption{Result details on real-world instances with multiple vehicles (Part 2)}
\label{tab:full2b}
\centering
\scriptsize % 调小字体
\resizebox{\columnwidth}{!}{
\begin{tabular}{rrrrrlr} 
\toprule
\multicolumn{1}{c}{\textbf{Ins}} & \multicolumn{1}{c}{\textbf{n}} & \multicolumn{1}{c}{$W_{Best}$} & \multicolumn{1}{c}{TT} & \multicolumn{1}{c}{$N_{veh}$} &  & \multicolumn{1}{c}{Gap}  \\ 
\midrule
\textbf{032} & 87  & 1205223.46 & 2011.92 & 20 & & 0.81 \\
\textbf{033} & 87  & 1053836.57 & 1747.60 & 18 & & 0.77 \\
\textbf{034} & 87  & 1399988.53 & 2308.77 & 24 & & 0.76 \\
\textbf{035} & 88  & 1068404.97 & 1783.02 & 18 & & 0.82 \\
\textbf{036} & 90  & 1276698.42 & 2106.07 & 22 & & 0.93 \\
\textbf{037} & 91  & 1206481.57 & 2021.59 & 20 & & 0.99 \\
\textbf{038} & 93  & 941496.96  & 1551.38 & 16 & & 1.15 \\
\textbf{039} & 98  & 1531762.13 & 2544.85 & 26 & & 1.30 \\
\textbf{040} & 98  & 1692423.57 & 2839.44 & 28 & & 1.28 \\
\textbf{041} & 104 & 1120009.66 & 1870.06 & 19 & & 1.53 \\
\textbf{042} & 105 & 1400651.05 & 2343.46 & 24 & & 0.80 \\
\textbf{043} & 106 & 1416699.78 & 2347.57 & 24 & & 1.69 \\
\textbf{044} & 110 & 1021367.59 & 1681.60 & 18 & & 1.91 \\
\textbf{045} & 110 & 1178598.16 & 2434.90 & 21 & & 2.15 \\
\textbf{046} & 110 & 1534117.14 & 2592.52 & 25 & & 2.30 \\
\textbf{047} & 114 & 1306986.80 & 2197.36 & 22 & & 2.73 \\
\textbf{048} & 115 & 1545978.28 & 2566.18 & 26 & & 2.73 \\
\textbf{049} & 116 & 1294564.47 & 1783.39 & 23 & & 2.87 \\
\textbf{050} & 117 & 1550340.75 & 2576.26 & 27 & & 2.85 \\
\textbf{051} & 119 & 1489288.28 & 2488.27 & 25 & & 3.00 \\
\textbf{052} & 121 & 1437003.39 & 2363.84 & 25 & & 3.14 \\
\textbf{053} & 121 & 1620065.26 & 2669.71 & 28 & & 2.92 \\
\textbf{054} & 123 & 1644541.98 & 2792.57 & 27 & & 3.45 \\
\textbf{055} & 127 & 1294030.20 & 2192.21 & 22 & & 3.99 \\
\textbf{056} & 128 & 1955192.84 & 3261.98 & 33 & & 4.33 \\
\textbf{057} & 129 & 1837813.30 & 3033.64 & 32 & & 4.95 \\
\textbf{058} & 135 & 1695431.80 & 2859.04 & 28 & & 5.36 \\
\textbf{059} & 136 & 1649242.21 & 2745.27 & 28 & & 5.21 \\
\textbf{060} & 143 & 1708512.35 & 2839.09 & 29 & & 4.60 \\
\textbf{061} & 145 & 1954030.69 & 3237.25 & 34 & & 5.03 \\
\textbf{062} & 165 & 2512379.48 & 4166.04 & 43 & & 5.24 \\ 
\midrule
\textbf{Avg} & \textbf{113} & \textbf{1469134.25} & \textbf{2450.22} & \textbf{25} & & \textbf{2.63} \\
\bottomrule
\end{tabular}}
\end{table}
